Improving Autoregressive Training with Dynamic Oracles

Many tasks within NLP can be framed as sequential decision problems, ranging from sequence tagging to text generation. However, for many tasks, the standard training methods, including maximum likelihood (teacher forcing) and scheduled sampling, suffer from exposure bias and a mismatch between metrics employed during training and inference. DAgger provides a solution to mitigate these problems, yet it requires a metric-specific dynamic oracle algorithm, which does not exist for many common metrics like span-based F1, ROUGE, and BLEU. In this paper, we develop these novel dynamic oracles and show they maintain DAgger's no-regret guarantee for decomposable metrics like span-based F1. We evaluate the algorithm's performance on named entity recognition (NER), text summarization, and machine translation (MT). While DAgger with dynamic oracle yields less favorable results in our MT experiments, it outperforms the baseline techniques in NER and text summarization.

==> tables/tex/avg_bleu_comparison.tex <==
\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c | c | c c c c}

        \multirow{2}{*}{\bf Epoch} & \multirow{1}{*}{\bf Ground Truth} &  \multicolumn{4}{c}{\bf Dynamic Oracle ($\Delta$ BLEU)}\\
         & \bf (BLEU) & \bf 5 & \bf 20 & \bf 90 & \bf 1000\\
        \hline
        2 & 72.10 &  +2.98 & +4.84 & +4.97 & +5.04 \\
        5 & 74.66 & +2.33 & +4.19 & +4.3 & +4.37 \\
        10 & 78.52 & +0.24 & 0.89 & +1.23 & +1.31 \\
        21 & 86.42 & -0.11 & +0.38 & +0.52 & +0.55 \\
    \end{tabular}
    }
    \caption{Average BLEU of ground truth supervision vs. dynamic oracle supervision. BLEU is averaged over all sentence in one batch. 5, 20, 90, 1000 are the beam sizes used for dynamic oracle.}
    \label{tab:BLEU_results}
\end{table}

==> tables/tex/teaser_comparison.tex <==
\begin{table}[h]
\resizebox{\columnwidth}{!}{%
    \centering
    \begin{tabular}{c  c  c  c}
    \bf Method & \bf Prefix & \bf Supervision & \bf Problem \\
    \toprule
    
    Teacher forcing & Gold & Gold & Exposure bias \\
    
    Scheduled Sampling & Gold + Model output & Gold & Wrong supervision \\
    
    DAgger & Gold + Model output & Dynamic oracle & Lacks dynamic oracle \\

    \end{tabular}
}
    \caption{Conceptual comparison of teacher forcing, scheduled sampling and DAgger.}
    \label{tab:teaser_comparison}
\end{table}


